Value-Guided KV Compression for LLMs via Approximated CUR Decomposition

Key-value (KV) cache compression has emerged as a critical technique for reducing the memory and latency overhead of autoregressive language models during inference. Prior approaches predominantly rely on query-key attention scores to rank and evict cached tokens, assuming that attention intensity correlates with semantic importance. However, this heuristic overlooks the contribution of value vectors, which directly influence the attention output. In this paper, we propose CurDKV, a novel, value-centric KV compression method that selects keys and values based on leverage scores computed from CUR matrix decomposition. Our approach approximates the dominant subspace of the attention output $softmax(QK^T)V$, ensuring that the retained tokens best preserve the model's predictive behavior. Theoretically, we show that attention score approximation does not guarantee output preservation, and demonstrate that CUR-based selection minimizes end-to-end attention reconstruction loss. Empirically, CurDKV achieves up to 9.6% higher accuracy than state-of-the-art methods like SnapKV and ChunkKV under aggressive compression budgets on LLaMA and Mistral, while maintaining compatibility with FlashAttention and Grouped Query Attention. In addition to improved accuracy, CurDKV reduces generation latency by up to 40% at high compression, offering a practical speed-accuracy tradeoff.

==> algorithm2.tex <==
\begin{algorithm}[t]
\caption{\adamethodname: Integration of \adamethodname\,  with AdaKV \citep{feng_ada-kv_2025}}
\label{alg:adacur-kv}
\KwIn{Key matrix $K \in \mathbb{R}^{g \times n \times d}$, Value matrix $V \in \mathbb{R}^{g \times n \times d}$, group budget $k$, Gaussian projection dim $r$, num\_sink $s$}
\KwOut{Compressed keys $K' \in \mathbb{R}^{g \times k \times d}$, values $V' \in \mathbb{R}^{g \times k \times d}$}


\end{algorithm}

